CompCap: Improving Multimodal Large Language Models with Composite Captions

How well can Multimodal Large Language Models (MLLMs) understand composite images? Composite images (CIs) are synthetic visuals created by merging multiple visual elements, such as charts, posters, or screenshots, rather than being captured directly by a camera. While CIs are prevalent in real-world applications, recent MLLM developments have primarily focused on interpreting natural images (NIs). Our research reveals that current MLLMs face significant challenges in accurately understanding CIs, often struggling to extract information or perform complex reasoning based on these images. We find that existing training data for CIs are mostly formatted for question-answer tasks (e.g., in datasets like ChartQA and ScienceQA), while high-quality image-caption datasets, critical for robust vision-language alignment, are only available for NIs. To bridge this gap, we introduce Composite Captions (CompCap), a flexible framework that leverages Large Language Models (LLMs) and automation tools to synthesize CIs with accurate and detailed captions. Using CompCap, we curate CompCap-118K, a dataset containing 118K image-caption pairs across six CI types. We validate the effectiveness of CompCap-118K by supervised fine-tuning MLLMs of three sizes: xGen-MM-inst.-4B and LLaVA-NeXT-Vicuna-7B/13B. Empirical results show that CompCap-118K significantly enhances MLLMs' understanding of CIs, yielding average gains of 1.7%, 2.0%, and 2.9% across eleven benchmarks, respectively.

==> tables/results_against_sota.tex <==
\begin{table}[t]
    \centering
    % \resizebox{\linewidth}{!}{
    \small
    \begin{tabular}{lcc}
    \toprule
        % Model & PT/SFT Data & MMB & MME\!& SEED & LLaVA$^\text{W}$  & QA$^\text{C}$  & VQA$^\text{D}$  & VQA$^\text{I}$  & WebSRC & MathV & OCRB & VQA$^\text{T}$  & Avg.\\
Model &
    PT/SFT \#Data& Avg. \\
\midrule
\rowcolor{lightgray}
\multicolumn{3}{l}{\emph{3B - 4B MLLMs}}\\
\midrule
Phi-3-vision~\citep{abdin2024phi} & 5B/$>$8.3M & \textbf{66.9}\\
xGen-MM-inst.-4B~\citep{xue2024xgen} & $>$25M/UNK. & \underline{60.2}\\
\rowcolor{isabelline}
xGen-MM-inst.-4B$^*$~\citep{xue2024xgen} & \cellcolor{lightblue}$>$25M/1M &  57.2\\
\rowcolor{isabelline}
CompCap-4B & \cellcolor{lightblue}$>$25M/1M  & {58.9}\\

\midrule
\rowcolor{lightgray}
\multicolumn{3}{l}{\emph{7B - 8B MLLMs}}\\
\midrule
ShareGPT4V-7B~\citep{chen2023sharegpt4v} & 1.2M/665K & 43.8\\
Qwen-VL-chat-7B~\citep{wang2024qwen2} & UNK./UNK. & 54.5\\
Cambrian-8B~\cite{tong2024cambrian} & 1.2M/7M & \textbf{65.9}\\
\rowcolor{isabelline}
LLaVA-NeXT-Vicuna-7B~\cite{liu2024llavanext} & \cellcolor{lightblue}558K/779K & 62.5\\
\rowcolor{isabelline}
CompCap-7B & \cellcolor{lightblue}558K/779K & \underline{64.5}\\
\midrule
\rowcolor{lightgray}
\multicolumn{3}{l}{\emph{13B MLLMs}}\\
\midrule
ShareGPT4V-13B~\citep{chen2023sharegpt4v} & 1.2M/665K  & 44.8\\
OmChat-v2.0-13B~\citep{zhao2024omchat} & $>$6.5B/20M & \textbf{75.0}\\
Cambrian-13B~\citep{tong2024cambrian} & 1.2M/7M & 67.2\\
\rowcolor{isabelline}
LLaVA-NeXT-Vicuna-13B~\citep{liu2024llavanext} & \cellcolor{lightblue}558K/779K & 65.6\\
\rowcolor{isabelline}
CompCap-13B & \cellcolor{lightblue}558K/779K & \underline{68.5}
\\
\bottomrule
\end{tabular}
% }
\caption{\textbf{Comparison against SOTA models in each size.}  We report the number of samples used for training (PT+SFT) to demonstrate SOTA MLLMs. The greater sign ``$>$'' indicates a lower bound of the number of samples, which is obtained by dividing the number of used tokens by the context window size 4K. We bold the best performance and underline the second best in each model size.}
\label{tab:main_result_sota}
\end{table}


==> tables/results_same_scale.tex <==
\begin{table*}[t]
    \centering
    % \resizebox{\linewidth}{!}{
    \small
    \begin{tabular}{lcccccccccccc}
    \toprule
        % Model & PT/SFT Data & MMB & MME\!& SEED & LLaVA$^\text{W}$  & QA$^\text{C}$  & VQA$^\text{D}$  & VQA$^\text{I}$  & WebSRC & MathV & OCRB & VQA$^\text{T}$  & Avg.\\
Model &
    \rotatebox{90}{\small{MMBench}} &
    \rotatebox{90}{\small{MME (norm)}} &
    \rotatebox{90}{\small{SEEDBench}} &
    \rotatebox{90}{\small{LLaVABench}} &
    \rotatebox{90}{\small{ChartQA}} &
    \rotatebox{90}{\small{DocVQA}} &
    \rotatebox{90}{\small{InfoVQA}} &
    \rotatebox{90}{\small{WebSRC}} &
    \rotatebox{90}{\small{MathVista}} &
    \rotatebox{90}{\small{OCRBench}} &
    \rotatebox{90}{\small{TextVQA}} &
    \rotatebox{90}{\small{Avg.}} \\
\midrule
\rowcolor{lightgray}
\multicolumn{13}{l}{\emph{4B MLLMs}}\\
\midrule
xGen-MM-inst.-4B$^*$~\citep{xue2024xgen} 
& 75.5          & 64.0          & 71.3          & 78.2          & 54.8          & 55.2          & 27.6          & 50.6          & 32.6          & 51.6          & 67.7          & 57.2\\
CompCap-4B 
& \textbf{76.2} & \textbf{64.7} & \textbf{71.6} & \textbf{81.0} & \textbf{57.4} & \textbf{58.1} & \textbf{27.9} & \textbf{55.8} & \textbf{35.0} & \textbf{52.7} & \textbf{67.9} & \textbf{58.9}\\

\midrule
\rowcolor{lightgray}
\multicolumn{13}{l}{\emph{7B MLLMs}}\\
\midrule
LLaVA-NeXT-Vicuna-7B~\cite{liu2024llavanext}  
& 67.6          & 66.3      & \textbf{71.2} & {72.4}        & 63.5          & 76.5          & 39.2          & 70.4          & 39.6          & 55.1          
& 65.2          & 62.5\\
CompCap-7B 
& \textbf{68.9} & \textbf{67.5}    & 70.5          & \textbf{75.5} & \textbf{68.9} & \textbf{77.6} & \textbf{40.8} & \textbf{73.7} & \textbf{41.7} & \textbf{58.5} 
& \textbf{65.6} & \textbf{64.5}\\
\midrule
\rowcolor{lightgray}
\multicolumn{13}{l}{\emph{13B MLLMs}}\\
\midrule
LLaVA-NeXT-Vicuna-13B~\citep{liu2024llavanext} 
& 68.9          & 68.8          & 71.9          & {77.1}        & 68.5          & 79.9      & 43.8          & 75.3          & 42.4          & 57.7          & 
67.6        & 65.6\\
CompCap-13B 
& \textbf{70.8} & \textbf{71.4} & \textbf{72.2} & \textbf{83.4} & \textbf{73.9} & \textbf{81.1}    & \textbf{47.0} & \textbf{79.3} & \textbf{45.0} & \textbf{61.4} & \textbf{67.8} & \textbf{68.5}
\\
\bottomrule
\end{tabular}
% }
\caption{\textbf{Evaluation on MLLM benchmarks.} For each model size, the two rows share the same MLLM architecture and PT dataset and are only difference in SFT data mixture (We retrain the SFT stage for xGen-MM-inst.-4B$^*$ for a fair comparison). Better performance are bolded in each model size.}
\label{tab:main_result_same_scale}
\end{table*}

